Robust Recommender System: A Survey and Future Directions

With the rapid growth of information, recommender systems have become integral for providing personalized suggestions and overcoming information overload. However, their practical deployment often encounters ``dirty'' data, where noise or malicious information can lead to abnormal recommendations. Research on improving recommender systems' robustness against such dirty data has thus gained significant attention. This survey provides a comprehensive review of recent work on recommender systems' robustness. We first present a taxonomy to organize current techniques for withstanding malicious attacks and natural noise. We then explore state-of-the-art methods in each category, including fraudster detection, adversarial training, certifiable robust training for defending against malicious attacks, and regularization, purification, self-supervised learning for defending against malicious attacks. Additionally, we summarize evaluation metrics and commonly used datasets for assessing robustness. We discuss robustness across varying recommendation scenarios and its interplay with other properties like accuracy, interpretability, privacy, and fairness. Finally, we delve into open issues and future research directions in this emerging field. Our goal is to provide readers with a comprehensive understanding of robust recommender systems and to identify key pathways for future research and development. To facilitate ongoing exploration, we maintain a continuously updated GitHub repository with related research: https://github.com/Kaike-Zhang/Robust-Recommender-System.

==> Section/2-Preliminary.tex <==
In this section, we begin by presenting mainstream recommendation tasks as foundational concepts. Following this, we provide a formal definition of robustness in the context of recommender systems. Lastly, we outline the taxonomy pertinent to this domain.



\subsection{Recommendation Tasks}
% To provide a clear understanding, we first introduce the symbols used in this survey in Table~\ref{tab:symbol}. 
To provide a clear understanding, we present the recommendation tasks associated with mainstream types of recommender systems. These mainstream recommendation tasks primarily fall into four categories: content-based recommender systems~\cite{Musto2022, Pazzani2007}, collaborative filtering-based recommender systems~\cite{Schafer2007, 10.1145/371920.372071}, sequential recommender systems~\cite{hidasi2016sessionbased, 10.1145/3109859.3109896}, and hybrid recommender systems~\cite{shani2005mdp, adomavicius2005toward}.

\textbf{Content-based Recommender Systems.} This type of recommender systems rely on the item's attributes (e.g., the genre of a movie or the theme of a book) to calculate similarity among items~\cite{Musto2022, zangerle2022evaluating}. If a user $u$ has expressed interest in an item $j$, and item $i$ is highly similar to item $j$, the model will likely recommend item $i$ to user $u$. One major advantage of content-based recommender systems is that they don't require data from other users, so they can often provide better recommendations for new items (also known as the item cold-start problem).

\textbf{Collaborative Filtering-based Recommender Systems (CF-based recommender systems).} This type of recommender systems base their recommendations on the behavior of users. They operate on the assumption that users who have similar behavior have similar preferences~\cite{zangerle2022evaluating}. Collaborative filtering can be categorized further into two types: memory-based (user-based~\cite{Schafer2007} and item-based~\cite{10.1145/371920.372071}) and model-based (e.g. matrix factorization)~\cite{ekstrand2011collaborative}. By examining these behavioral patterns, CF-based recommender systems can unveil unexpected item associations, exemplified by the pairing of beer and diapers.
% However, CF-based recommender systems have issues with scalability and the cold-start problem, where it is difficult to make recommendations for new users or items due to a lack of historical data.

\textbf{Sequential Recommender Systems.} This type of recommender systems focus on the order or sequence of user-item interactions~\cite{Schafer2007, 10.1145/371920.372071}. They consider the temporal dynamics of user behavior, where recent interactions have more influence on the current recommendation than the older ones. This kind of recommender systems is particularly useful in domains where user preferences shift over time, such as music or news recommendations. Sequential recommendation models often use techniques such as Markov Chains, Recurrent Neural Networks (RNNs), or Transformer-based models for the task~\cite{sun2019bert4rec}.

\textbf{Hybrid Recommender Systems.} Hybrid recommender systems combine two or more recommendation strategies in different ways to benefit from their complementary advantages~\cite{zangerle2022evaluating}. For example, a hybrid system might use collaborative filtering as a base but fall back on content-based methods when collaborative data is sparse, thus alleviating the cold-start problem associated with CF-based recommender systems~\cite{burke2002hybrid}. Hybrid methods can be implemented in several ways: by making predictions based on the weighted sum of different recommendation techniques, by switching between recommendation techniques based on user-context, by using one technique to improve the predictions of another, and so on. These systems have been shown to provide more accurate recommendations than single-method systems in various domains.

Regardless of the specific recommendation task, a general form can be used to represent the learning objectives of the recommender system. Suppose we have a set of $M$ users, denoted by $\mathcal{U}$, a set of $N$ items, denoted by $\mathcal{I}$, and a rating set $\mathcal{R}$, containing feedback $r_{u,i}$ of user $u \in \mathcal{U}$ for item $i \in \mathcal{I}$. The collected user-item interactions are represented by $\mathcal{D}$, where $(u, i, r_{u,i}) \in \mathcal{D}$. Our goal is to learn a parametric model $f:\mathcal{U} \times \mathcal{I} \rightarrow \mathcal{R}$ from $\mathcal{D}$ that minimizes the following objective function:
\begin{equation}
    \begin{aligned}
        % \mathcal{L} = \mathbb{E}_\mathcal{D}[\psi(f(u,i),r_{u,i})]
        % \mathcal{L}(\mathcal{D}) = \sum_{u \in \mathcal{U}} \sum_{i \in \mathcal{I}} \psi(f(u,i),r_{u,i}).
        \mathcal{L}(\mathcal{D}) = \sum_{(u, i, r_{u,i}) \in \mathcal{D}} \psi(f(u,i),r_{u,i}),
    \end{aligned}
    \label{eq:org_l}
\end{equation}
where $\psi$ is the error function used to measure the distance between the predicted and ground truth labels. In order to facilitate the search for the corresponding meaning of the symbol, we provide the corresponding meaning of the symbol used in this survey in Table~\ref{tab:symbol}.

In the actual training process, we typically divide the collected data $\mathcal{D}$ into a training set $\mathcal{D}^+$ and a test set $\mathcal{D}^-$.
After training on $\mathcal{D}^+$ through $\mathcal{L}(\mathcal{D}^+)$ mentioned in Equation~\ref{eq:org_l}, we obtain an recommender systems model denoted as $f_{\mathcal{D}^+}$. 
% To evaluate its performance, we use various metrics $M$ to assess the effectiveness of the recommender systems model on the test set $\mathcal{D}^-$ (see details in Section~\ref{5-Eva}). 

% However, in practice, we cannot obtain the unobserved data $\mathcal{D}^-$. Therefore, we typically divide the observed data $\mathcal{D}$ into a training set and a test set to simulate the training and evaluation processes of recommender systems. For the sake of clarity, we will use $\mathcal{D}$ to represent the training set and $\mathcal{D}^-$ to represent the test set throughout the remainder of this survey.


% \begin{figure}[t]%
% \centering
% \includegraphics[width=0.9\textwidth]{Figs/transductive.pdf}
% \caption{Comparison of traditional models and recommendation systems (recommender systems): In traditional models, perturbations can occur in both training and test data; In recommender systems, perturbations are only introduced in the training data.}\label{trans_rs}
% \end{figure}
\input{Table/symbol}

\subsection{Definition of Robustness in Recommender System}
\label{definition_sec}
The term ``robustness'' initially described three essential characteristics of a parameterized model: efficiency, stability, and non-breakdown~\cite{huber1981robust}. Efficiency requires the model to be sufficiently accurate. Stability means minor deviations from the model's assumptions should only minimally impact performance. Non-breakdown denotes that large deviations should not catastrophically affect performance. With the development of deep learning, robustness now generally refers to a predictor's ability to maintain performance given minor data perturbations~\cite{fawzi2017robustness}, including the data perturbations in the training phase and test phase:

\begin{itemize}
    \item \textbf{Data Perturbations in Training Phase}: This refers to instances where the training data contains part of pollution, often called poisoning attacks~\cite{jagielski2018manipulating, tian2022comprehensive}. In recommender systems, this aims to manipulate the training data (e.g., inject fake users) to degrade performance or promote/nuke items~\cite{tang2020revisiting, christakopoulou2019adversarial}.
    \item \textbf{Data Perturbations in Test Phase}: This refers to instances where the test data is contaminated, typically known as evasion attacks~\cite{biggio2013evasion, bhagoji2017dimensionality}. In recommender systems, this aims to manipulate the test input to mislead recommendations.
\end{itemize}

Although both types exist, test phase perturbations place stronger restrictions on models, requiring inductive abilities. Therefore, different from robustness in other fields like CV or NLP, almost all existing research for recommender systems' robustness on robustness in recommender systems assumes that data perturbations only occur in the training phase~\cite{15_zhang2017robust, 58_gunawardana2012evaluating, 47_oh2022rank, 60_o2004collaborative, tang2020revisiting}. Hence, in this survey, we only discuss the robustness of the first scenario, i.e., data perturbations in the training phase.

% It is important to note that although both types of data perturbations exist, perturbations in the test phase impose stronger restrictions on the recommendation model, i.e. the model is required to have an inductive ability. Therefore, almost all research assumes that data perturbations only occur in the training phase~\cite{15_zhang2017robust, 58_gunawardana2012evaluating, 47_oh2022rank, 60_o2004collaborative, tang2020revisiting}. Hence, in this survey, we only discuss the robustness of the first scenario, i.e., data perturbations in the training phase.

% Several works related to robustness in recommender systems define it as the stability of performance under data pollution or contamination~\cite{58_gunawardana2012evaluating,47_oh2022rank,60_o2004collaborative,15_zhang2017robust}.

\begin{figure}[t]%
\centering
\includegraphics[width=0.9\textwidth]{Figs/category_legend.pdf}
\vspace{-0.3cm}
\\
\subfigure[User-item interaction graph]{
\includegraphics[width=0.2775\textwidth]{Figs/category_1.pdf}
}
\subfigure[with malicious attack]{
\includegraphics[width=0.3424\textwidth]{Figs/category_2.pdf}
\label{cat_attack}
}
\subfigure[with noisy interaction]{
\includegraphics[width=0.2801\textwidth]{Figs/category_3.pdf}
\label{cat_noise}
}
\caption{User-item interaction graph with malicious attack and natural noise.}
\end{figure}

Considering these factors, we propose that the robustness of a recommender system should be measured by its ability to maintain stable model output in the presence of perturbations to the training data. We formalize this with the following definition of robustness for recommender systems:

\begin{definition}[$(\epsilon, \varepsilon)$-Robust Recommender Systems]
Given a recommendation model $f$, a dataset $\mathcal{D} = \{\mathcal{D}^{+}, \mathcal{D}^{-}\}$, a bounded perturbation $\Delta$ such that $|\Delta|_p \leq \epsilon$, and an acceptable error threshold $\varepsilon$, if
\begin{equation}
    |f_{\mathcal{D}^+}(\mathcal{D}^-) - f_{\mathcal{D}^++\Delta}(\mathcal{D}^-)| \leq \varepsilon,
\end{equation}
where $f_{\mathcal{D}^{+}}$ and $f_{\mathcal{D}^{+}+\Delta}$ are model $f$ trained on the original and perturbed data respectively, then model $f$ is considered $(\epsilon, \varepsilon)$-robust.
\end{definition}


% The robustness of a recommendation model $f$ under the bounded perturbation $\Delta$ for the dataset $\mathcal{D} = \{\mathcal{D}^+, \mathcal{D}^-\}$ has a negative correlation with the difference in the model's predictions on $\mathcal{D}^-$ when $f$ is trained with or without perturbations.

% These perturbations are not associated with the specific recommender systems model, but rather the integrity of the data itself. 
% This form of perturbation necessitates that the input of the recommender systems model contains user or item features, not merely their IDs.

% In recommendation scenarios, mainstream research typically assumes that the user set $\mathcal{U}$ and item set $\mathcal{I}$ are fixed. Consequently, data perturbations generally occur only during the training stage, as illustrated in Figure~\ref{trans_rs}. On the other hand, test time attacks require attackers to hack into normal users' accounts and change their preferences, which is a cybersecurity issue and beyond the scope of recommender systems' robustness~\cite{tang2020revisiting}.
% \begin{definition}[Robustness of recommender systems]
% \label{def_robust}
% For a recommendation model $f$, dataset $\mathcal{D}$, a bounded perturbation $\Delta$, and a specific threshold $\varepsilon$, if
% \begin{equation}
%     \delta(M, M') \leq \varepsilon,
% \end{equation}
% where $\delta(\cdot)$ is a difference function, and $M_{f_{D}}$ and $M_{f_{D+\Delta}}$ are the performances of model $f$ trained on clean data $D$ and perturbed data $D+\Delta$, respectively, then $f$ is considered robust.
% \end{definition}






\subsection{Taxonomy of Robustness in Recommender System}



% \input{Table/category}



% For malicious attacks, attackers often aim to promote or nuke specific items, or damage the performance of recommender systems. However, adversarial scenarios often restrict the attackers' abilities to manipulate a user's historical behavior. There are typically two types of attacks in recommendation scenarios, item side information modification and fake user injection, as shown in Figure~\ref{cat_attack}. The former is the instance of attackers manipulating item information with the aim of artificially augmenting the popularity of their products, as depicted in the top of Figure~\ref{cat_attack}. The latter is the instance of resorting to introducing fake users with the intention of inflating or deflating the popularity of certain items or degrading the overall performance of the recommender systems, as shown in the bottom of Figure~\ref{cat_attack}.

Recommender systems function as highly interactive platforms, making them vulnerable to various forms of abnormal data. These anomalies can originate from malicious activities such as injecting fake users and tampering with item information, or from natural noise which typically arises due to human errors or ambiguities in user behavior.

For malicious attacks, attackers often aim to promote/nuke specific items or damage the performance of recommender systems. Generally, adversarial scenarios often restrict the attackers' abilities to manipulate a user's historical behavior. There are typically two types of attacks in recommendation scenarios, as shown in Figure~\ref{cat_attack}:
\begin{itemize}
\item Item side information modification: Attackers manipulate item side information to artificially augment the popularity of specific items~\cite{cohen2021black}, as depicted in the top of Figure~\ref{cat_attack}.
\item Fake user injection~(shilling attack): Introducing fake users to inflate or deflate the exposure of certain items or degrade the overall performance of the recommender systems~\cite{tang2020revisiting, christakopoulou2019adversarial}, as shown in the bottom of Figure~\ref{cat_attack}.
\end{itemize}
It is essential to note that, even with limitations on potential attack, several defense mechanisms against interaction-level attacks have been proposed in the literature~\cite{7_yuan2020exploring, 42_chen2022adversarial, 30_yue2022defending, 9_liu2020certifiable}. For a comprehensive understanding, these defense methodologies will be elaborated upon in the subsequent sections, particularly in section~\ref{adv-on-int}.

Natural noise mainly stems from user-generated factors such as human errors, uncertainty, and ambiguity in user behavior~\cite{20_yera2016fuzzy}. For instance, it may manifest in the historical interactions between users and items, such as misclicks or gifts reflecting others' tastes, as illustrated in Figure~\ref{cat_noise}. Note that, noise can also occur in user or item side information, such as incorrect personal information or item tags. However, due to the paucity of research addressing these types of noise in the context of recommender systems~\cite{53_liu2021concept}, Figure~\ref{cat_noise} does not show this category.

To enhance the robustness of recommender systems, it is essential to differentiate between the various types of abnormal data. Accordingly, we categorize the robustness of recommender systems into two primary types based on the nature of these anomalies:

\begin{figure}
    \centering
    \resizebox{0.8\textwidth}{!}{\input{Tex_Graph/Category2}}
    \caption{A lookup graph for the reviewed methods for robustness in recommender systems.}
    \label{fig:category}
\end{figure}

\begin{itemize}
    \item \textbf{Robustness against malicious attacks}: This involves strategies to mitigate injected users or falsified item data. Approaches can be broadly divided into three categories: fraudster detection~\cite{28_wu2012hysad,16_zhang2020gcn,14_cao2020adversarial}, adversarial training~\cite{4_he2018adversarial,2_tang2019adversarial,30_yue2022defending}, and certifiable robust training~\cite{9_liu2020certifiable}. Fraudster detection involves identifying fraudsters within the training data and minimizing their influence on model training, either by eliminating them or assigning them lower weights. Adversarial training aims to bolster the model's robustness against malicious attacks by positively introducing small perturbations during the training process. Certifiable robust training involves training the model to function optimally under worst-case perturbations that can be certified.
    \item \textbf{Robustness against natural noise}: This involves methods designed to mitigate the impact of noisy interactions. Techniques can be classified into three categories: regularization~\cite{15_zhang2017robust,39_chen2022denoising}, purification~\cite{43_wang2021denoising,27_tian2022learning}, and self-supervised learning~\cite{46_shenbin2020recvae,35_wang2022learning}. Regularization methods typically introduce a regularization term (e.g., R1-norm regularization~\cite{15_zhang2017robust}) in the loss function, causing the model to downplay the noise in the data. Purification techniques strive to identify and rectify noise in user-item interactions to improve the performance and robustness of the recommender systems. Self-supervised learning approaches endeavor to mitigate noise through generative-based methods (e.g., Denoising Autoencoder~\cite{8_li2015deep, 46_shenbin2020recvae}) and contrastive-based methods (e.g., contrastive learning~\cite{27_tian2022learning, 37_chen2022intent}).
\end{itemize}


The taxonomy of publications on recommender systems' robustness is presented in Figure~\ref{fig:category}.


% by leveraging the inherent structure of the data or by creating variations of existing data as auxiliary information.


==> Section/5-subsection/1-Eva_RS.tex <==
recommender systems are evaluated using various metrics that measure their performance in terms of accuracy, ranking quality, relevance, and other factors. Here, we introduce some widely used evaluation metrics, presenting both their descriptions and formalized definitions:

\begin{itemize}
\item \textbf{Mean Absolute Error (MAE)}: MAE measures the average absolute difference between the predicted ratings and the actual ratings:
\begin{equation}
    \begin{aligned}
        \mathrm{MAE} = \frac{1}{|\mathcal{D}|} \sum_{(u,i) \in \mathcal{D}} |\hat{r}_{u,i} - r_{u,i}|,
    \end{aligned}
\end{equation}
where $r_{u,i}$ is the actual rating, and $\hat{r}_{u,i}$ is the predicted rating. MAE is particularly useful for assessing the prediction accuracy of rating-based recommender systems.

\item \textbf{Root Mean Square Error (RMSE)}: RMSE measures the square root of the average squared difference between the predicted ratings and the actual ratings:
\begin{equation}
    \begin{aligned}
        \mathrm{RMSE} = \sqrt{\frac{1}{|\mathcal{D}|} \sum_{(u,i) \in \mathcal{D}} (\hat{r}_{u,i} - r_{u,i})^2}.
    \end{aligned}
\end{equation}
RMSE is another accuracy metric for rating-based recommender systems, emphasizing larger errors compared to MAE.

\item \textbf{Recall$@k$}: Recall$@k$ measures the proportion of relevant items that are included in the top-k recommended items:
\begin{equation}
    \begin{aligned}
        \mathrm{Recall}@k = \frac{1}{|\mathcal{U}|} \sum_{u \in \mathcal{U}} \frac{|\hat{L}_u@k \cap L_u|}{|L_u|},
    \end{aligned}
\end{equation}
where $L_u$ is the ground truth preferred list for user $u$, and $\hat{L}_u@k$ is the top-k recommendation list given by recommender systems. Recall$@k$ assesses the ability of recommender systems to cover relevant items within the top-k recommendations.


\item \textbf{Precision$\bm{@k}$}: Precision$@k$ measures the proportion of relevant items among the top-k recommended items:
\begin{equation}
    \begin{aligned}
        \mathrm{Precision}@k = \frac{1}{|\mathcal{U}|} \sum_{u \in \mathcal{U}}  \frac{|\hat{L}_u@k \cap L_u|}{k}.
    \end{aligned}
\end{equation}
Precision$@k$ is particularly important for recommender systems which focuses on recommending the most relevant items to users within a limited set of top-k items.

\item \textbf{F1-score$\bm{@k}$}: F1-score$@k$ is the harmonic mean of precision$@k$ and recall$@k$, providing a balanced evaluation of both metrics:
\begin{equation}
    \begin{aligned}
        \mathrm{F1}-\mathrm{score}@k = 2 \cdot \frac{\mathrm{Precision}@k \cdot \mathrm{Recall}@k}{\mathrm{Precision}@k + \mathrm{Recall}@k}.
    \end{aligned}
\end{equation}
F1-score$@k$ is especially useful when considering both the quality of top-k recommendations and the coverage of relevant items.

\item \textbf{Normalized Discounted Cumulative Gain (NDCG$\bm{@k}$)}: NDCG$@k$ measures the ranking quality of the top-k recommended items, considering the relevance of each item and penalizing lower-ranked relevant items:
\begin{equation}
    \begin{aligned}
        \mathrm{NDCG}@k = \frac{\mathrm{DCG}@k}{\mathrm{IDCG}@k},
    \end{aligned}
\end{equation}
where $DCG@k = \sum_{i=1}^k \frac{2^{rel_i} - 1}{\log_2(i+1)}$ is the Discounted Cumulative Gain, $rel_i$ is the relevance of the item at position $i$, and IDCG$@k$ is the ideal DCG$@k$, which is the maximum possible DCG for $L_u$. NDCG$@k$ is particularly important for recommender systems which emphasizes the quality of the ranking order of recommended items.

% \item \textbf{Hit Ratio$\bm{@k}$ (HR$\bm{@k}$) for single item}: It measures the proportion of users for whom at least one test item is included in the top-k recommendation list:
% \begin{equation}
%     \begin{aligned}
%         % HR@k = \frac{\sum_{u \in \mathcal{U}} |\hat{L}_u@k \cap L_u|}{\sum_{u \in \mathcal{U}} |L_u|}
%         \mathrm{HR}@k = \frac{\#\mathit{hits}}{\#\mathit{users}},
%     \end{aligned}
%     \label{eq:hr_1}
% \end{equation}
% where $\#\mathit{hits}$ is the number of users whose test item appears in the recommendation list.

\item \textbf{Hit Ratio$\bm{@k}$ (HR$\bm{@k}$) for top-$\bm{k}$ recommendation}: It measures the fraction of test items that appear in the top-k recommendation list relative to all test items:
\begin{equation}
    \begin{aligned}
        \mathrm{HR}@k = \frac{\sum_{u \in \mathcal{U}} |\hat{L}_u@k \cap L_u|}{\sum_{u \in \mathcal{U}} |L_u|}.
    \end{aligned}
    \label{eq:hr_2}
\end{equation}
It's worth noting that when the test set contains only a single item, Eq.\ref{eq:hr_2} simplifies to $\mathrm{HR}@k = \#\mathit{hits} / \#\mathit{users}$, where $\#\mathit{hits}$ is the number of users whose test item appears in the recommendation list. HR$@k$ is useful for assessing the overall effectiveness of recommender systems in satisfying users' preferences within a limited set of top-k recommendations.
\end{itemize}

These evaluation metrics capture different aspects of recommender systems' performance, and researchers typically use several of them to assess the overall quality and effectiveness of their models. By employing these metrics, researchers can gain insights into the strengths and weaknesses of their recommender systems and make informed decisions on how to improve their models to better cater to users' needs and preferences.

==> Table/category.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
% \begin{table}[htbp]
%   \renewcommand{\arraystretch}{1.5}
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{|m{0.12\textwidth}|m{0.1\textwidth}|m{0.1\textwidth}|m{0.08\textwidth}m{0.08\textwidth}m{0.1\textwidth}|m{0.2\textwidth}|}
%     \hhline{|-------|}
%     % \cline{1-2}
%     \multicolumn{3}{|c|}{\multirow{3}*{Category}} &\multicolumn{3}{c|}{Resist Perturbations on}                           &\multirow{3}*{\centering Publication} \\
%     \hhline{|~~~---~|}
%     \multicolumn{3}{|c|}{}        &\multicolumn{2}{c|}{Side Information}                     &\multirow{2}*{Interaction}  &\multicolumn{1}{c|}{} \\
%     \hhline{~~~--~~}
%     \multicolumn{3}{|c|}{}        &\multicolumn{1}{c|}{-user}   &\multicolumn{1}{c|}{-item}  &\multicolumn{1}{c|}{}       &\multicolumn{1}{c|}{} \\
%     \hline
%     \multirow{5}{0.15\textwidth}{Robustness against Malicious Attack} &\multirow{3}{0.1\textwidth}{Adversarial Training} &\multicolumn{1}{l|}{with Parameters} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
%     \hhline{~~-----}
%     \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{}  &\multicolumn{1}{l|}{with Content Data} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{publications} \\
%     \hhline{~~-----}
%     \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{}  &\multicolumn{1}{l|}{with Interaction} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
%     \hhline{~------}
%     \multicolumn{1}{|c|}{}    & \multicolumn{2}{l|}{Fraudster Detection} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
%     \hhline{~------}
%     \multicolumn{1}{|c|}{}    & \multicolumn{2}{l|}{Purification} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
%     \hline
%     \multirow{4}{0.15\textwidth}{Robustness against Natural Noise} & \multicolumn{2}{l|}{Regularization} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
%     \hhline{~------}
%     \multicolumn{1}{|c|}{}    & \multicolumn{2}{l|}{Purification} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
%     \hhline{~------}
%     \multicolumn{1}{|c|}{}    &\multirow{2}{0.1\textwidth}{Self-supervised Learning}    &\multicolumn{1}{l|}{Contrastive Learning} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
%     \hhline{~~-----}
%     \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{}  &\multicolumn{1}{l|}{Edge Masking} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
%     \hline
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%


% % % Table generated by Excel2LaTeX from sheet 'Sheet2'
% % \begin{table}[htbp]
% %   \renewcommand{\arraystretch}{1.5}
% %   \centering
% %   \caption{Add caption}
% %     % \begin{tabular}{|m{0.12\textwidth}m{0.1\textwidth}|m{0.1\textwidth}|m{0.08\textwidth}m{0.08\textwidth}m{0.1\textwidth}|m{0.2\textwidth}|}
% %     \noindent\begin{tabularx}{0.9\textwidth}{|r|r|r|c|c|c|r|}
% %     \hhline{|-------|}
% %     \multicolumn{3}{|c|}{\multirow{3}*{Category}} &\multicolumn{3}{c|}{Resist Perturbations on}                           &\multirow{3}*{\centering Publication} \\
% %     \hhline{|~~~---~|}
% %     \multicolumn{3}{|c|}{}        &\multicolumn{2}{c|}{Side Information}                     &\multirow{2}*{Interaction}  &\multicolumn{1}{c|}{} \\
% %     \hhline{~~~--~~}
% %     \multicolumn{3}{|c|}{}        &\multicolumn{1}{c|}{-user}   &\multicolumn{1}{c|}{-item}  &\multicolumn{1}{c|}{}       &\multicolumn{1}{c|}{} \\
% %     \hline
% %     \multirow{5}{0.15\textwidth}{Robustness against Malicious Attack} &\multirow{3}{0.1\textwidth}{Adversarial Training} &\multicolumn{1}{l|}{with Parameters} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
% %     \hhline{~~-----}
% %     \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{}  &\multicolumn{1}{l|}{with Content Data} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{publications} \\
% %     \hhline{~~-----}
% %     \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{}  &\multicolumn{1}{l|}{with Interaction} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
% %     \hhline{~------}
% %     \multicolumn{1}{|c|}{}    & \multicolumn{2}{l|}{Fraudster Detection} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
% %     \hhline{~------}
% %     \multicolumn{1}{|c|}{}    & \multicolumn{2}{l|}{Purification} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
% %     \hline
% %     \multirow{4}{0.15\textwidth}{Robustness against Natural Noise} & \multicolumn{2}{l|}{Regularization} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
% %     \hhline{~------}
% %     \multicolumn{1}{|c|}{}    & \multicolumn{2}{l|}{Purification} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
% %     \hhline{~------}
% %     \multicolumn{1}{|c|}{}    &\multirow{2}{0.1\textwidth}{Self-supervised Learning}    &\multicolumn{1}{l|}{Contrastive Learning} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
% %     \hhline{~~-----}
% %     \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{}  &\multicolumn{1}{l|}{Edge Masking} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{*} &\multicolumn{1}{c|}{publications} \\
% %     \hline
% %     % \end{tabular}%
% %     \end{tabularx}
% %   \label{tab:addlabel}%
% % \end{table}%


% \begin{sidewaystable}[htbp]
%     \renewcommand{\arraystretch}{1.2}
%     \centering
%     \caption{A lookup table for the reviewed methods for robustness in recommender systems.}
%     \begin{tabular}{ccp{0.12\textwidth}ccc>{\raggedright\arraybackslash}p{0.3\textwidth}}
%         \toprule
%         % \multicolumn{3}{c}{\multirow{3}{0.1\textwidth}{Category}} &\multicolumn{3}{c}{Resist Perturbations on} & \multirow{3}{0.2\textwidth}{\centering Publication} \\
%         \multicolumn{3}{c}{\multirow{3}{0.1\textwidth}{Category}} &\multicolumn{3}{c}{Resist Perturbations on} & \multirow{3}{0.2\textwidth}{\centering Publication} \\
%         \cmidrule{4-6}
%         % & & &\multicolumn{2}{c}{Side Information} &\multirow{2}{0.1\textwidth}{Interaction} & \\
%         % & & &-user &-item & & \\
%         & & &\multirow{1}{0.06\textwidth}{\centering User} &\multirow{1}{0.06\textwidth}{\centering Item} &\multirow{1}{0.06\textwidth}{\centering Inter-} & \\
%         & & &Profile &Profile &action & \\
%         \midrule
%         \multirow{7}{0.1\textwidth}[-2em]{\centering Robustness against Malicious Attack} &\multirow{4}{0.1\textwidth}[-1.5em]{Adversarial Training on} &Parameters &\checkmark &\checkmark &\checkmark &\cite{1_du2018enhancing,4_he2018adversarial,5_yuan2019adversarial,6_yuan2019adversarial,24_chen2019adversarial,32_li2020adversarial,40_ye2023towards, 66_tran2019adversarial}\\
%         \cmidrule{3-7}
%         & &User Profile &\checkmark & & &\cite{17_wu2021fight} \\
%         \cmidrule{3-7}
%         & &Item Profile & & \checkmark & &\cite{2_tang2019adversarial,3_anelli2021study} \\
%         \cmidrule{3-7}
%         & &Interaction & & &\checkmark &\cite{42_chen2022adversarial, 30_yue2022defending, 7_yuan2020exploring} \\
%         \cmidrule{2-7}
%         &\multirow{3}{0.1\textwidth}[-0.8em]{Fraudster Detection} &before Training &\checkmark & & &\cite{10_zhang2015catch,11_yang2016re,12_yang2017spotting,13_aktukmak2019quick,25_zhang2014hht,26_zhou2014detection,28_wu2012hysad,29_beutel2014cobafi,33_chung2013betap,45_zou2013belief,49_liu2020recommending,50_lee2012shilling,51_cao2013shilling,52_zhou2016svm} \\
%         % &\multicolumn{2}{l}{Fraudster Detection} &\checkmark & &
%         \cmidrule{3-7}
%         & &in Training &\checkmark & & &\cite{16_zhang2020gcn} \\
%         \cmidrule{3-7}
%         & &after Training &\checkmark & & &\cite{14_cao2020adversarial} \\
%         \cmidrule{2-7}
%         &\multicolumn{2}{l}{Certifiable Robustness} &\checkmark &\checkmark &\checkmark &\cite{9_liu2020certifiable} \\
%         \midrule
%         \multirow{4}{0.1\textwidth}[-1.5em]{\centering Robustness against Natural Noise} &\multicolumn{2}{l}{Regularization} & & &\checkmark &\cite{15_zhang2017robust,39_chen2022denoising} \\
%         \cmidrule{2-7}
%         &\multicolumn{2}{l}{Purification} & & &\checkmark &\cite{20_yera2016fuzzy, 31_gao2022self, 41_toledo2015correcting, 43_wang2021denoising, 44_bian2021denoising, 53_liu2021concept, 56_wang2021implicit, 27_tian2022learning, 39_chen2022denoising, 54_qin2021world} \\
%         \cmidrule{2-7}
%         &\multirow{2}{0.1\textwidth}[-0.5em]{Self-supervised Learning} &Contrastive Learning & & &\multirow{1}*[-0.5em]{\checkmark} &\multirow{1}*[-0.5em]{\cite{23_liu2021contrastive, 27_tian2022learning, 34_yang2022knowledge, 35_wang2022learning, 36_wu2021self, 37_chen2022intent, 54_qin2021world, 40_ye2023towards}} \\
%         \cmidrule{3-7}
%         & &Edge Masking & & &\checkmark &\cite{8_li2015deep,21_wu2016collaborative,38_zheng2021multi,46_shenbin2020recvae,55_strub2015collaborative} \\
%         \bottomrule
%     \end{tabular}%
%     \label{tab:category}%
% \end{sidewaystable}

% \begin{sidewaystable}[htbp]
%     \renewcommand{\arraystretch}{1.2}
%     \centering
%     \caption{A lookup table for the reviewed methods for robustness in recommender systems.}
%     \begin{tabular}{ccp{0.12\textwidth}ccc>{\raggedright\arraybackslash}p{0.3\textwidth}}
%         \toprule
%         % \multicolumn{3}{c}{\multirow{3}{0.1\textwidth}{Category}} &\multicolumn{3}{c}{Resist Perturbations on} & \multirow{3}{0.2\textwidth}{\centering Publication} \\
%         \multicolumn{3}{c}{\multirow{3}{0.1\textwidth}{Category}} &\multicolumn{3}{c}{Resist Perturbations on} & \multirow{3}{0.2\textwidth}{\centering Publication} \\
%         \cmidrule{4-6}
%         % & & &\multicolumn{2}{c}{Side Information} &\multirow{2}{0.1\textwidth}{Interaction} & \\
%         % & & &-user &-item & & \\
%         & & &\multirow{1}{0.06\textwidth}{\centering User} &\multirow{1}{0.06\textwidth}{\centering Item} &\multirow{1}{0.06\textwidth}{\centering Inter-} & \\
%         & & &Profile &Profile &action & \\
%         \midrule
%         \multirow{7}{0.1\textwidth}[-6em]{\centering Robustness against Malicious Attack} &\multirow{4}{0.1\textwidth}[-2.5em]{Adversarial Training on} & \multirow{1}*[-1em]{Parameters} 
%         & \multirow{1}*[-1em]{\checkmark} &\multirow{1}*[-1em]{\checkmark}  &\multirow{1}*[-1em]{\checkmark}  &\cite{1_du2018enhancing,4_he2018adversarial,5_yuan2019adversarial,6_yuan2019adversarial,24_chen2019adversarial,32_li2020adversarial,40_ye2023towards, 66_tran2019adversarial}\\
%         \cmidrule{3-7}
%         & &User Profile &\checkmark & & &\cite{17_wu2021fight} \\
%         \cmidrule{3-7}
%         & &Item Profile & & \checkmark & &\cite{2_tang2019adversarial,3_anelli2021study} \\
%         \cmidrule{3-7}
%         & &\multirow{1}*[-0.5em]{Interaction} & & &\multirow{1}*[-0.5em]{\checkmark} &\cite{42_chen2022adversarial, 30_yue2022defending, 7_yuan2020exploring, 9_liu2020certifiable} \\
%         \cmidrule{2-7}
%         &\multirow{3}{0.1\textwidth}[-3.5em]{Fraudster Detection} &\multirow{1}*[-3em]{Pre-training} &\multirow{1}*[-3em]{\checkmark} & & &\cite{10_zhang2015catch,11_yang2016re,12_yang2017spotting,13_aktukmak2019quick,25_zhang2014hht,26_zhou2014detection,28_wu2012hysad,29_beutel2014cobafi,33_chung2013betap,45_zou2013belief,49_liu2020recommending,50_lee2012shilling,51_cao2013shilling,52_zhou2016svm} \\
%         % &\multicolumn{2}{l}{Fraudster Detection} &\checkmark & &
%         \cmidrule{3-7}
%         & &In-raining &\checkmark & & &\cite{16_zhang2020gcn} \\
%         \cmidrule{3-7}
%         & &Post-training &\checkmark & & &\cite{14_cao2020adversarial} \\
%         \cmidrule{2-7}
%         &\multicolumn{2}{l}{Certifiable Robustness} &\checkmark &\checkmark &\checkmark &\cite{9_liu2020certifiable} \\
%         \midrule
%         \multirow{4}{0.1\textwidth}[-5em]{\centering Robustness against Natural Noise} &\multicolumn{2}{l}{Regularization} & & &\checkmark &\cite{15_zhang2017robust,39_chen2022denoising} \\
%         \cmidrule{2-7}
%         &\multicolumn{2}{l}{\multirow{1}*[-2.5em]{Purification}} & & &\multirow{1}*[-2.5em]{\checkmark} &\cite{20_yera2016fuzzy, 31_gao2022self, 41_toledo2015correcting, 43_wang2021denoising, 44_bian2021denoising, 53_liu2021concept, 56_wang2021implicit, 27_tian2022learning, 39_chen2022denoising, 54_qin2021world} \\
%         \cmidrule{2-7}
%         &\multirow{2}{0.1\textwidth}[-2.5em]{Self-supervised Learning} & \multirow{1}*[-2em]{Contrastive Learning} & & &\multirow{1}*[-2em]{\checkmark} &\cite{23_liu2021contrastive, 27_tian2022learning, 34_yang2022knowledge, 35_wang2022learning, 36_wu2021self, 37_chen2022intent, 54_qin2021world, 40_ye2023towards} \\
%         % &\multirow{1}*[-0.5em]{\cite{23_liu2021contrastive, 27_tian2022learning, 34_yang2022knowledge, 35_wang2022learning, 36_wu2021self, 37_chen2022intent, 54_qin2021world, 40_ye2023towards}} \\
%         \cmidrule{3-7}
%         & &\multirow{1}*[-1.5em]{Edge Masking} & & &\multirow{1}*[-1.5em]{\checkmark} &\cite{8_li2015deep,21_wu2016collaborative,38_zheng2021multi,46_shenbin2020recvae,55_strub2015collaborative} \\
%         \bottomrule
%     \end{tabular}%
%     \label{tab:category}%
% \end{sidewaystable}

\begin{table}[t]
    \renewcommand{\arraystretch}{1.2}
    \centering
    \caption{A lookup table for the reviewed methods for robustness in recommender systems.}
    \begin{tabular}{ccp{0.15\textwidth}ccc>{\raggedright\arraybackslash}p{0.3\textwidth}}
        \toprule
        % \multicolumn{3}{c}{\multirow{3}{0.1\textwidth}{Category}} &\multicolumn{3}{c}{Resist Perturbations on} & \multirow{3}{0.2\textwidth}{\centering Publication} \\
        \multicolumn{3}{c}{\multirow{3}{0.1\textwidth}{Category}} &\multicolumn{3}{c}{Resist Perturbations on} & \multirow{3}{0.2\textwidth}{\centering Publication} \\
        \cmidrule{4-6}
        % & & &\multicolumn{2}{c}{Side Information} &\multirow{2}{0.1\textwidth}{Interaction} & \\
        % & & &-user &-item & & \\
        & & &\multirow{1}{0.06\textwidth}{\centering User} &\multirow{1}{0.06\textwidth}{\centering Item} &\multirow{1}{0.06\textwidth}{\centering Inter-} & \\
        & & &Profile &Profile &action & \\
        \midrule
        \multirow{7}{0.1\textwidth}[-3em]{\centering Robustness against Malicious Attack} &\multirow{3}{0.1\textwidth}[-1em]{Fraudster Detection} &\multirow{1}*[-0.5em]{Pre-processing} &\multirow{1}*[-0.5em]{\checkmark} & & &\cite{28_wu2012hysad, 61_zhang2012meta, 50_lee2012shilling, 45_zou2013belief, 51_cao2013shilling, 25_zhang2014hht, 63_zhang2014detection, 26_zhou2014detection, 10_zhang2015catch, 64_zhou2015shilling, 11_yang2016re, 52_zhou2016svm, 12_yang2017spotting, 13_aktukmak2019quick, 49_liu2020recommending} \\
        % &\multicolumn{2}{l}{Fraudster Detection} &\checkmark & &
        \cmidrule{3-7}
        & &In-processing &\checkmark & & &\cite{16_zhang2020gcn} \\
        \cmidrule{3-7}
        & &Post-processing &\multirow{1}*{\checkmark} & & &\multirow{1}*{\cite{14_cao2020adversarial}} \\
        \cmidrule{2-7}
         &\multirow{4}{0.1\textwidth}[-1em]{Adversarial Training on} & \multirow{1}*{Parameters} 
        & \multirow{1}*{\checkmark} &\multirow{1}*{\checkmark}  &\multirow{1}*{\checkmark}  &\cite{4_he2018adversarial,1_du2018enhancing,5_yuan2019adversarial,6_yuan2019adversarial,24_chen2019adversarial,66_tran2019adversarial,32_li2020adversarial,40_ye2023towards}\\
        \cmidrule{3-7}
        & &User Profile &\checkmark & & &\cite{17_wu2021fight} \\
        \cmidrule{3-7}
        & &Item Profile & & \checkmark & &\cite{2_tang2019adversarial,3_anelli2021study} \\
        \cmidrule{3-7}
        & &\multirow{1}*{Interaction} & & &\multirow{1}*{\checkmark} &\cite{7_yuan2020exploring, 9_liu2020certifiable, 42_chen2022adversarial, 30_yue2022defending} \\
        \cmidrule{2-7}
        &\multicolumn{2}{l}{Certifiable Robustness} &\checkmark &\checkmark &\checkmark &\cite{9_liu2020certifiable} \\
        \midrule
        \multirow{3}{0.1\textwidth}[-1.5em]{\centering Robustness against Natural Noise} &\multicolumn{2}{l}{\multirow{1}*{Regularization}} & & &\multirow{1}*{\checkmark} &\cite{15_zhang2017robust,39_chen2022denoising} \\
        \cmidrule{2-7}
        &\multicolumn{2}{l}{\multirow{1}*[-0.5em]{Purification}} & & &\multirow{1}*[-0.5em]{\checkmark} &\cite{71_pham2013preference, 20_yera2016fuzzy, 43_wang2021denoising, 44_bian2021denoising, 53_liu2021concept, 54_qin2021world, 56_wang2021implicit, 27_tian2022learning, 31_gao2022self, 39_chen2022denoising, 70_xie2022denoising, 40_ye2023towards} \\
        \cmidrule{2-7}
        &\multicolumn{2}{l}{\multirow{1}*[-0.5em]{Self-supervised Learning}} &\multirow{1}*[-0.5em]{\checkmark} &\multirow{1}*[-0.5em]{\checkmark} &\multirow{1}*[-0.5em]{\checkmark} &\cite{67_zhou2020s3, 8_li2015deep, 55_strub2015collaborative, 21_wu2016collaborative, 46_shenbin2020recvae, 23_liu2021contrastive, 36_wu2021self, 38_zheng2021multi, 27_tian2022learning, 34_yang2022knowledge, 35_wang2022learning, 37_chen2022intent} \\
        \midrule
        \midrule
        \multirow{3}{0.1\textwidth}[-1em]{\centering Evaluation} &\multicolumn{2}{l}{\multirow{1}*[-0.5em]{Metrics Offset}} &\multirow{1}*[-0.5em]{-} &\multirow{1}*[-0.5em]{-} &\multirow{1}*[-0.5em]{-} 
        &\cite{48_deldjoo2020dataset, 59_shrestha2021empirical, 1_du2018enhancing, 2_tang2019adversarial, 3_anelli2021study, 4_he2018adversarial, 5_yuan2019adversarial, 6_yuan2019adversarial, 7_yuan2020exploring, 8_li2015deep, 16_zhang2020gcn, 17_wu2021fight, 18_vinagre2019statistically, 23_liu2021contrastive, 27_tian2022learning, 30_yue2022defending,35_wang2022learning, 37_chen2022intent, 39_chen2022denoising, 40_ye2023towards, 55_strub2015collaborative}
        % \setcitestyle{open={},close={}}
        % &[\cite{2_tang2019adversarial, 24_chen2019adversarial} $,\dots,$ \cite{59_shrestha2021empirical, 55_strub2015collaborative} $,\dots$]
        % \setcitestyle{open={[},close={]}}
        \\
        % 3 也是多攻击指标偏移指标
        % 4 用的 NDCG 偏移 23 37 40
        % 5 用的 HR 偏移 6 7 27 39
        % 8 用的 RMSE 16
        % 17 用的 新提的指标 近似计算 rank 偏移
        %  
        \cmidrule{2-7}
        &\multicolumn{2}{l}{\multirow{1}*{Output Offset}} &- &- &- &\cite{47_oh2022rank, 57_shriver2019evaluating} \\
        \cmidrule{2-7}
        &\multicolumn{2}{l}{\multirow{1}*{Certifiable Robustness}} &- &- &- &\cite{9_liu2020certifiable} \\
        \bottomrule
    \end{tabular}%
    \label{tab:category}%
\end{table}
